Locality-based Graph Reordering for Processing Speed-Ups and Impact of Diameter

Graph analysis involves a high number of random memory access patterns. Earlier research has shownthat the cache miss latency is responsible for more than half of the graph processing time, with the CPU execution having the smaller share. There has been significant study on decreasing the CPU computing time for example, by employing better cache prefetching and replacement policies. In thispaper, we study the various methods that do so by attempting to decrease the CPU cache miss ratio.Graph Reordering attempts to exploit the power-law distribution of graphs -- few sparsely-populated vertices in the graph have high number of connections -- to keep the frequently accessed vertices together locally and hence decrease the cache misses. However, reordering the graph by keeping the hot vertices together may affect the spatial locality of the graph, and thus add to the total CPU compute time.Also, we also need to have a control over the total reordering time and its inverse relation with thefinal CPU execution timeIn order to exploit this trade-off between reordering as per vertex hotness and spatial locality, we introduce the light-weight Community-based Reordering. We attempt to maintain the community-structureof the graph by storing the hot-members in the community locally together. The implementation also takes into consideration the impact of graph diameter on the execution time. We compare our implementation with other reordering implementations and find a significantly better result on five graph processing algorithms: BFS, CC, CCSV, PR and BC. Lorder achieved speed-up of upto 7x and an average speed-up of 1.2x as compared to other reordering algorithms

==> Chapters/Chapter_6.tex <==
\clearpage
\chapter{Conclusion}




==> Chapters/Chapter_7.tex <==
\clearpage
\chapter{Experimental Results and Observations}

\section{Inductive-Invariant Generation using Logical Cone Clustering}
In the first set of experiments, we applied the proposed algorithm for invariant generation on ITC' 99 and ISCAS' 89 benchmark circuits.

\subsection{ITC' 99 Benchmark Circuits}
Table 7.1 illustrates the characteristics of ITC' 99 circuits along with $TargetSize$ and $N_{cluster}$ used for logical cone clustering. The last column in Table 7.1 shows the number of valid clusters which were iteratively used for invariant generation. \\

 \begin{table}[H]
\centering
\caption{$TargetSize$ and $N_{cluster}$ used for clustering in ITC' 99 Benchmark circuits}
\label{tab:rank_based}
\scalebox{1}{
\begin{tabular}{ |p{1.3cm}|p{1.6cm}|p{1.75cm}|p{1.1cm}|p{2cm}|p{2.1cm}|p{1.6cm}|}
\hline
\textbf{Circuit} & \textbf{Primary Inputs} & \textbf{Primary Outputs} & \textbf{Flip-Flops} & \textbf{TargetSize} & \textbf{Number of clusters} & \textbf{Valid clusters} \\ \hline
b01 & 2 & 2 & 5 & 5 & 1 & 0* \\ \hline
b02 & 1 & 1 & 4 & 4 & 1 & 1 \\ \hline
b03 & 4 & 4 & 30 & 5 & 5 & 2 \\ \hline
b04 & 11 & 8 & 66 & 7 & 7 & 3 \\ \hline
b05 & 1 & 36 & 34 & 5 & 5 & 5 \\ \hline
b06 & 2 & 6 & 9 & 3 & 3 & 1 \\ \hline
b07 & 1 & 8 & 49 & 7 & 7 & 6 \\ \hline
b08 & 9 & 4 & 21 & 4 & 4 & 4 \\ \hline
b09 & 1 & 1 & 28 & 5 & 5 & 5 \\ \hline
b10 & 11 & 6 & 17 & 3 & 3 & 3 \\ \hline
b11 & 7 & 6 & 31 & 5 & 5 & 5 \\ \hline
b12 & 5 & 6 & 121 & 11 & 11 & 8 \\ \hline
b13 & 10 & 10 & 53 & 7 & 7 & 3 \\ \hline
b14 & 32 & 54 & 245 & 13 & 18 & 11 \\ \hline
b15 & 37 & 69 & 417 & 13 & 32 & 24 \\ \hline
b17 & 39 & 96 & 864 & 13 & 66 & 11* \\ \hline
b20 & 32 & 22 & 490 & 13 & 37 & 20 \\ \hline
b21 & 33 & 22 & 429 & 13 & 33 & 31 \\ \hline
\end{tabular}}
\end{table} 
In the case of b01, a repeated flip-flop was removed to generate a valid cluster. In b04 and b10, default parameter selection did not give any valid clusters. Therefore, a lower value for $TargetSize$ and $N_{cluster}$ was selected. In the case of b17, clusters having 19 inputs were selected for invariant generation by providing their initial 13 inputs to LUT.\\

Table 7.2 shows the results pertaining to the best performing cluster for ITC' 99 circuits. The best performing cluster was selected based on the percentage of unreachable states in the extracted invariant. In these experiments, all the flip-flops have been initialized to zero in the initial state and ABC \cite{ref_18} has been used as the QBF solver. 

\begin{table}[H]
\centering
\caption{Inductive Invariant Generation for ITC' 99 Benchmark circuits with the proposed algorithm}
\label{tab:rank_based}
\scalebox{1.1}{
\begin{tabular}{ |p{1.5cm} |p{2cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
\hline
\textbf{Circuit} &
\textbf{Number of inputs to LUT} &   \textbf{Unreachable States} & \textbf{Reachable States} & \textbf{Percentage of Unreachable States} \\ \hline
b01 & 4 & 6 & 10 & 37.5 \\ \hline
b02 & 4 & 8 & 8 & 50  \\ \hline
b03 & 10 & 512 & 512 & 50 \\ \hline
b04 & 7 & 16 & 112 & 12.5 \\ \hline
b05 & 7 & 72 & 56 & 56.25 \\ \hline
b06 & 3 & 1 & 7 & 12.5 \\ \hline
b07 & 7 & 120 & 8 & 93.75 \\ \hline
b08 & 9 & 271 & 241 & 52.93 \\ \hline
b09 & 8 & 155 & 101 & 60.55 \\ \hline
b10 & 7 & 26 & 102 & 20.31 \\ \hline
b11 & 5 & 18 & 14 & 56.25 \\ \hline
b12 & 11 & 1076 & 972 & 52.54 \\ \hline
b13 & 11 & 1808 & 240 & 88.28 \\ \hline
b14 & 13 & 8191 & 1 & 99.99 \\ \hline
b15 & 14 & 8192 & 8192 & 50 \\ \hline
b17 & 13 & 7527 & 665 & 91.88 \\ \hline
b20 & 13 & 8191 & 1 & 99.99 \\ \hline
b21 & 13 & 6847 & 1345 & 83.58 \\ \hline
\end{tabular}}
\end{table} 

\textbf{Observations:} We have been able to generate invariants having unreachable states in all the circuits considered in the experiment. \\
 For circuits like b14 and b20, we have been able to obtain invariants in which almost all the states are unreachable. In such cases, the state space has been pruned to a significant extent.\\
 For b17, the clusters having 13 inputs did not yield any effective invariant. Therefore, clusters having 19 inputs were selected for invariant generation by providing their initial 13 inputs to LUT.
 For other circuits, the state space has been pruned significantly as we have been able to obtain invariants having almost half of all the states as unreachable states. \\



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.45]{Images/plot1.PNG}
    \caption{Percentage of unreachable states obtained for ITC' 99 Benchmark circuits with the proposed algorithm}
    \label{fig: Software model}
\end{figure}   

\newpage

\subsection{ISCAS' 89 Benchmark Circuits}
Table 7.3 illustrates the characteristics of ISCAS' 89 circuits along with $TargetSize$ and $N_{cluster}$ used for logical cone clustering. The last column in Table 7.3 shows the number of valid clusters which were iteratively used for invariant generation. \\

\begin{table}[H]
\centering
\caption{$TargetSize$ and $N_{cluster}$ used for clustering in ISCAS' 89 Benchmark circuits}
\label{tab:rank_based}
\scalebox{1}{
\begin{tabular}{ |p{1.3cm}|p{1.6cm}|p{1.75cm}|p{1.1cm}|p{2cm}|p{2.1cm}|p{1.6cm}|}
\hline
\textbf{Circuit} & \textbf{Primary Inputs} & \textbf{Primary Outputs} & \textbf{Flip-Flops} & \textbf{TargetSize} & \textbf{Number of clusters} & \textbf{Valid clusters} \\ \hline
s298 & 3 & 6 & 14 & 3 & 3 & 3 \\ \hline
s344 & 9 & 11 & 15 & 3 & 3 & 3  \\ \hline
s349 & 9 & 11 & 15 & 3 & 3 & 3 \\ \hline
s382 & 3 & 6 & 21 & 4 & 4 & 4 \\ \hline
s400 & 3 & 6 & 21 & 4 & 4 & 4 \\ \hline
s444 & 3 & 6 & 21 & 4 & 4 & 4  \\ \hline
s510 & 19 & 7 & 6 & 6 & 1 & 1   \\ \hline
s526 & 3 & 6 & 21 & 4 & 4 & 1   \\ \hline
s641 & 35 & 24 & 19 & 4 & 4 & 4   \\ \hline
s713 & 35 & 23 & 19 & 4 & 4 & 4  \\ \hline
s820 & 18 & 19 & 5 & 5 & 1 & 1   \\ \hline
s832 & 18 & 19 & 5 & 5 & 1 & 1   \\ \hline
s953 & 16 & 23 & 29 & 5 & 5 & 5   \\ \hline
s9234 & 19 & 22 & 228 & 13 & 17 & 17   \\ \hline
s13207.1 & 62 & 152 & 638 & 13 & 49 & 49   \\ \hline
s38417 & 28 & 106 & 1636 & 13 & 125 & 125   \\ \hline
s38584 & 12 & 278 & 1452 & 13 & 111 & 111   \\ \hline
\end{tabular}}
\end{table}

Table 7.4 shows the results pertaining to the best performing cluster for ISCAS' 89 circuits. The best performing cluster was selected based on the percentage of unreachable states in the extracted invariant. In these experiments, all the flip-flops have been initialized to zero in the initial state and ABC \cite{ref_18} has been used as the QBF solver.

\begin{table}[H]
\centering
\caption{Inductive Invariant Generation for ISCAS' 89 Benchmark circuits with the proposed algorithm}
\label{tab:rank_based}
\scalebox{1.1}{
\begin{tabular}{ |p{1.5cm} |p{2cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
\hline
\textbf{Circuit} &
\textbf{Number of inputs to LUT} &   \textbf{Unreachable States} & \textbf{Reachable States} & \textbf{Percentage of Unreachable States} \\ \hline
s298 & 6 & 46 & 18 & 71.88   \\ \hline
s344 & 6 & 16 & 48 & 25   \\ \hline
s349 & 6 & 16 & 48 & 25   \\ \hline
s382 & 6 & 24 & 40 & 37.5   \\ \hline
s400 & 6 & 24 & 40 & 37.5   \\ \hline
s444 & 6 & 24 & 40 & 37.5   \\ \hline
s510 & 6 & 17 & 47 & 26.56   \\ \hline
s526 & 9 & 474 & 38 & 92.58  \\ \hline
s641 & 4 & 6 & 10 & 37.5   \\ \hline
s713 & 4 & 6 & 10 & 37.5   \\ \hline
s820 & 5 & 7 & 25 & 21.88  \\ \hline
s832 & 5 & 7 & 25 & 21.88   \\ \hline
s953 & 5 & 17 & 15 & 53.13  \\ \hline
s9234 & 6 & 63 & 1 & 98.44   \\ \hline
s13207.1 & 13 & 7936 & 256 & 96.88   \\ \hline
s38417 & 13 & 8168 & 24 & 99.71   \\ \hline
s38584 & 13 & 8176 & 16 & 99.80   \\ \hline

\end{tabular}}
\end{table} 

\textbf{Observations:} We have been able to generate invariants having unreachable states in all the circuits. \\
 For larger circuits like s38417 and s38584, we have been able to obtain invariants in which almost all the states are unreachable. In such cases, the state space has been pruned to a significant extent.\\
 For other circuits, the state space has been pruned significantly as we have been able to obtain invariants having almost $40 \%$ of all the states as unreachable states. \\



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.45]{Images/plot2.PNG}
    \caption{Percentage of unreachable states obtained for ISCAS' 89 Benchmark circuits with the proposed algorithm}
    \label{fig: Software model}
\end{figure}   




\section{Comparison with X-value based Analysis}
In this section, we have compared results obtained through our proposed algorithm with those obtained through X-value based analysis. X-value based analysis is the current state of the art in invariant extraction \cite{ref_16}. The maximum size of the valid cluster considered for our iterative algorithm has been fixed as the number of flip-flops which should be provided as inputs to LUT in order of X-value based ranking discussed previously. In these experiments, all the flip-flops have been initialized to zero in the initial state. An effective invariant in this context means an invariant with at least one unreachable state.

\newpage

\subsection{ITC' 99 Benchmark Circuits}
Table 7.5 shows the comparison between results obtained through our proposed algorithm with those obtained through X-value based analysis on ITC' 99 benchmark circuits. In these experiments, all the flip-flops have been initialized to zero in the initial state and ABC \cite{ref_18} has been used as the QBF solver.


\begin{table}[H]
\centering
\caption{Comparison with Benchmark Results for ITC' 99 Benchmark circuits}
\label{tab:rank_based}
\scalebox{0.9}{
\begin{tabular}{ |p{1.3cm} |p{1.6cm}|p{2.5cm}|p{2cm}|p{2.5cm}|p{3cm}|}
\hline
& \multicolumn{4}{c|}{\textbf{Proposed Algorithm}} &   \\ \hline
\textbf{Circuit} &
\textbf{Number of LUT inputs} &   \textbf{Unreachable States} & \textbf{Reachable States} &
\textbf{Effective Invariant ?? (Proposed Algorithm)} &
\textbf{Effective Invariant ?? (X-value based Analysis)}
\\ \hline
b01 & 4 & 6 & 10 & YES & YES \\ \hline
b02 & 4 & 8 & 8 & YES & YES\\ \hline
b03 & 10 & 512 & 512 & YES & YES \\ \hline
b04 & 7 & 16 & 112 & \textbf{YES}
& \textbf{NO}\\ \hline
b05 & 7 & 72 & 56 & YES & YES \\ \hline
b06 & 3 & 1 & 7 & YES & YES \\ \hline
b07 & 7 & 120 & 8 & \textbf{YES} 
& \textbf{NO}\\ \hline
b08 & 9 & 271 & 241 & YES & YES \\ \hline
b09 & 8 & 155 & 101 & 
\textbf{YES} & \textbf{NO} \\ \hline
b10 & 7 & 26 & 102 & YES & YES \\ \hline
b11 & 5 & 18 & 14 & \textbf{YES}   & \textbf{NO}\\ \hline
b12 & 11 & 1076 & 972 & \textbf{YES}  & \textbf{NO} \\ \hline
b13 & 11 & 1808 & 240 & YES & YES \\ \hline
b14 & 13 & 8191 & 1 & \textbf{YES}
& \textbf{NO}\\ \hline
b15 & 14 & 8192 & 8192 & \textbf{YES}
& \textbf{NO}\\ \hline
b17 & 13 & 7527 & 665 & \textbf{YES}
& \textbf{NO}\\ \hline
b20 & 13 & 8191 & 1 & \textbf{YES}
& \textbf{NO}\\ \hline
b21 & 13 & 6847 & 1345 & \textbf{YES}
& \textbf{NO}\\ \hline
\end{tabular}}
\end{table} 
    

    
\textbf{Observation:} In 10 out of the 18 circuits, where X-value based analysis failed to generate an effective invariant, we obtained effective inductive invariants through the proposed algorithm.

\newpage

\subsection{ISCAS' 89 Benchmark Circuits}
Table 7.6 shows the comparison between results obtained through our proposed algorithm with those obtained through X-value based analysis on ISCAS' 89 benchmark circuits. In these experiments, all the flip-flops have been initialized to zero in the initial state and ABC \cite{ref_18} has been used as the QBF solver.

\begin{table}[H]
\centering
\caption{Comparison with Benchmark Results for ISCAS' 89 Benchmark circuits}
\label{tab:rank_based}
\scalebox{0.9}{
\begin{tabular}{ |p{1.3cm} |p{1.6cm}|p{2.5cm}|p{2cm}|p{2.5cm}|p{3cm}|}
\hline
& \multicolumn{4}{c|}{\textbf{Proposed Algorithm}} &   \\ \hline
\textbf{Circuit} &
\textbf{Number of LUT inputs} &   \textbf{Unreachable States} & \textbf{Reachable States} &
\textbf{Effective Invariant ?? (Proposed Algorithm)} &
\textbf{Effective Invariant ?? (X-value based Analysis)}
\\ \hline
s298 & 6 & 46 & 18 & YES & YES \\ \hline
s344 & 6 & 16 & 48 & \textbf{YES} & \textbf{NO} \\ \hline
s349 & 6 & 16 & 48 & \textbf{YES} & \textbf{NO} \\ \hline
s382 & 6 & 24 & 40 & YES & YES \\ \hline
s400 & 6 & 24 & 40 & YES & YES \\ \hline
s444 & 6 & 24 & 40 & YES & YES \\ \hline
s510 & 6 & 17 & 47 & YES & YES\\ \hline
s526 & 9 & 474 & 38 & YES & YES \\ \hline
s641 & 4 & 6 & 10 & \textbf{YES} & \textbf{NO}\\ \hline
s713 & 4 & 6 & 10 & \textbf{YES} & \textbf{NO}\\ \hline
s820 & 5 & 7 & 25 & YES & YES \\ \hline
s832 & 5 & 7 & 25 & YES & YES \\ \hline
s953 & 5 & 17 & 15 & YES & YES \\ \hline
s9234 & 6 & 63 & 1 & \textbf{YES}
& \textbf{NO}\\ \hline
s13207.1 & 13 & 7936 & 256 & YES & YES \\ \hline
s38417 & 13 & 8168 & 24 & \textbf{YES}
& \textbf{NO}\\ \hline
s38584 & 13 & 8176 & 16 & YES & YES \\ \hline
\end{tabular}}
\end{table} 

\textbf{Observation:} In 6 out of the 17 circuits, where X-value based analysis failed to generate an effective invariant, we obtained effective inductive invariants through the proposed algorithm.

\newpage

\section{Time Taken for Logical Cone Clustering}
The logical cone clustering for most of the circuits in ISCAS' 89 and ITC' 99 benchmarks is completed within a minute. However, for circuits having a large number of gates, it takes time in order of 30 minutes. The graph in Figure 7.3.1 shows the time taken for logical cone clustering on a machine having 16GB RAM and Intel i7 processor and operating at 2.80 GHz. The graph shows the time taken on some representative circuits taken from both ITC' 99 and ISCAS' 89 benchmark circuits.



\begin{figure} [H]
    \centering
    \includegraphics[scale=1.3]{Images/g1.PNG}
    \caption{Time required for clustering (in minutes) for target cluster size of 13}
    \label{fig: Software model}
\end{figure}
 



==> Chapters/Chapter_8.tex <==
\clearpage
\chapter{Conclusions and Scope for Future Work}
We have shown that our proposed algorithm based on logical cone clustering can find effective inductive invariants having a significant proportion of unreachable states in almost all of the ISCAS' 89 and ITC' 99 circuits considered in various experiments. Our proposed algorithm has been able to find invariants with unreachable states even for those circuits in ISCAS' 89 and ITC' 99 benchmarks where previous methods of flip-flop selection have failed. This can lead to significant pruning of state-space for these benchmark circuits and reduction in computational effort required for solving various problems in formal analysis and logic synthesis.\\

Some of the ideas presented in this dissertation can be investigated further. The proposed algorithm for invariant extraction can be made robust by the inclusion of other netlist parameters. Machine Learning based approaches should also be investigated for flip-flop clustering. Having obtained inductive invariants with a significant number of unreachable states, these invariants can be used for logic optimization \cite{ref_16}. In the context of model checking, further research is needed in cases where the QBF equation is UNSAT after 15 inputs to LUT to establish the confirmation. Eventually, the unreachable states obtained through inductive invariants can be incorporated into algorithms used for VLSI testing.



==> Template/SOOA.tex <==
\clearpage
\thispagestyle{empty}
\section*{Declaration of Academic Ethics}
\label{sec:SOOA}
\vspace{-1.5cm}

% Statement of original authorship - Needs to be in German
% see also here: https://www.wiso.uni-koeln.de/sites/fakultaet/dokumente/PA/formulare/eidesstattliche_erklaerung.pdf

\subparagraph{\textnormal{I hereby declare that the dissertation titled \textbf{\textquotedblleft Enhanced Reachability Analysis Using Inductive Invariant Computation\textquotedblright} represents my ideas in my own words. In all occurrences where ideas or words or diagrams are taken from books/papers/electronic media, I have adequately cited and acknowledged the sources. I declare that I have adhered to all principles of academic honesty and integrity and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will result in disciplinary action as per the norms of the Institute and can also evoke legal action from the sources which have thus not been properly acknowledged or from whom proper permission has not been taken.}}

% \subparagraph{\textnormal{
% I also declare that I have adhered to all principles of academic honesty and integrity and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will be cause for disciplinary action by the Institute and can also evoke penal action from the sources which have thus not been properly cited or from whom proper permission has not been taken when needed.}}
\vspace{1cm}

\noindent

\vspace{3cm}
\noindent
\textbf{\thesisauthor{}\\
Roll No. 160070031\\
Department of Electrical Engineering\\
Indian Institute of Technology Bombay}

\vspace{0.5cm}
\noindent
Date: 25/6/2021 


==> Template/dissertation.tex <==



% \Declaration% Add a gap in the Contents, for aesthetics
\thispagestyle{empty}
 \begin{center}
{\Large { Acknowledgements}} \\
 \vspace{0.2in}
 This is to certify that the dissertation titled\\
 \vspace{0.1in}
 {\bf Enhanced Reachability Analysis Using Inductive Invariant Computation} \\
 \vspace{0.2in}
 by \\
\vspace{0.1in}
 {\bf Abhijeet Aanand} \\ (160070031) \\
 \vspace{0.2in}
 is approved for the degree of {\bf Bachelor \& Master of Technology in Electrical Engineering}.\\
 \vspace{0.5in}

 \end{center}
 \vspace*{0.2in}


 %%\line(1,0){100}


%\begin{figure}[h]
 %%  \includegraphics[scale=0.76]{./Figures1/approval_harsh.jpg}
    % \caption{Decision Tree of adder circuit}.
   % \label{fig:approval}
%\end{figure}




\newpage
\clearpage

